If You Must Choose Among Your Children, Pick the Right One

Given a simplicial complex $K$ and an injective function $f$ from the vertices of $K$ to $\mathbb{R}$, we consider algorithms that extend $f$ to a discrete Morse function on $K$. We show that an algorithm of King, Knudson and Mramor can be described on the directed Hasse diagram of $K$. Our description has a faster runtime for high dimensional data with no increase in space.

==> body/append-cancel.tex <==
\section{A New Cancellation Algorithm}
\begin{algorithm}
    \caption{\cleankid}\label{alg: Child Clean Up}
    \begin{algorithmic}[1]
	
	\Require $\gvf \in K$, injective fcn.\ $f_0: K_0\rightarrow \mathbb{R}$
        \Ensure a refined GVF consistent with $f_0$

        \State{$\hasseK_\C \gets $ Construct upward Hasse diagram from $\C \in K$}

        \State $\tails^* \gets \tails$, $\heads^* \gets \heads$, $\criticals^*
        \gets \criticals$, $\matches^* \gets \matches$

        \For {$i = \dim{\hasseK_\C}$ to $1$}
        \label{line:cchild-downd}

        \For{$\sigma \in \hasseKI{i}$}\label{line:cchild-ltor}

        \If{$\sigma$ is assigned}
        \State {\bf continue}
        \EndIf

        \If{$\sigma$ is a left-right match}

        \State {Add $\rchild{\sigma}$ to $\tails^*$; Add $\sigma$ to $\heads^*$}

        \State{Add $(\rchild{\sigma},\sigma)$ to $r^*$}
        \label{line:cchild-defro}
        
        \State {Remove $\rchild{\sigma}$ and $\sigma$ from $\criticals$}

        \State Mark $\sigma$ and $\rchild{\sigma}$ as assigned

        \Else

        \State Keep $\sigma$ in $C$\label{line:cchild-addc}
        \State Mark $\sigma$ as assigned

        \EndIf

        \EndFor
        \EndFor

        \State{Keep any unassigned vertex in $\criticals$}
        \label{line:cchild-leftovers}\\

        \Return $(\tails^*, \heads^*, \criticals^*, r^*)$
        \label{line:cchild-return}

    \end{algorithmic}
\end{algorithm}

